PruneForget: Joint Unlearning and Pruning of Vision Models

Machine unlearning and model pruning are increasingly coupled in the real world. Models must support unlearning requests, e.g., for safety concerns, while also meeting requirements in latency and memory budget. Until recently, existing works have studied each aspect as an independent problem, e.g., running unlearning and pruning sequentially. In this work, we show that unlearning and pruning are naturally aligned and should be solved jointly to be made aware of each other. Intuitively, parameters that encode information of the unlearned samples are natural pruning targets, as unlearning and pruning both call for the "deletion" of such parameters. We propose PruneForget, a method that uses the unlearn set as a guide for pruning, so that unlearning and pruning mutually benefit each other. Extensive experiments on image classifiers and generative models show that PruneForget removes the influence of the unlearned samples while producing a more compact model with reduced inference cost. It achieves a negligible performance gap relative to an oracle that retrains from scratch for unlearning and then prunes.

==> includes/macros.tex <==
\makeatletter
\renewcommand{\paragraph}{%
    \@startsection{paragraph}{4}%
    {\z@}{0.3ex \@plus 1ex \@minus .1ex}{-1em}%
    {\normalfont\normalsize\bfseries}%
}
\makeatother

% Usage
% \myparagraph{PARAGRAPH_TITLE}
\newcommand{\myparagraph}[1]{\vspace*{0pt}{\bf #1}}


% Usage
% \best{BEST_NUMBER}
% \second{SECOND_NUMBER}
\newcommand{\best}[1]{\textbf{#1}}
\newcommand{\second}[1]{\underline{#1}}


% Shortcut for \begin \end equations
\newcommand{\beas}{\begin{eqnarray*}}
\newcommand{\eeas}{\end{eqnarray*}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bes}{\begin{equation*}}
\newcommand{\ees}{\end{equation*}}
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}

% \newtheorem{proposition}{Prop}
% \newtheorem{lemma-ap}{Lemma}
% \newtheorem{definition}{Definition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{claim}{Claim}
% \newtheorem{claim-ap}{Claim}
% \newtheorem{program}{Program}
% \newtheorem{property}{Property}

\makeatletter
\usepackage{xspace}
\def\@onedot{\ifx\@let@token.\else.\null\fi\xspace}
\DeclareRobustCommand\onedot{\futurelet\@let@token\@onedot}
\def\sp{space}

\newcommand{\figref}[1]{Fig\onedot~\ref{#1}}
\newcommand{\equref}[1]{Eq\onedot~\eqref{#1}}
\newcommand{\secref}[1]{Sec\onedot~\ref{#1}}
\newcommand{\tabref}[1]{Tab\onedot~\ref{#1}}
\newcommand{\thmref}[1]{Theorem~\ref{#1}}
\newcommand{\prgref}[1]{Program~\ref{#1}}
% \providecommand{\algref}{}
% \renewcommand{\algref}[1]{Alg.~\ref{#1}} % to avoid clash with some other package
\newcommand{\clmref}[1]{Claim~\ref{#1}}
\newcommand{\lemref}[1]{Lemma~\ref{#1}}
\newcommand{\ptyref}[1]{Property\onedot~\ref{#1}}
\newcommand{\vsp}{\csname v\sp \endcsname}
\newcommand{\hsp}{\csname h\sp \endcsname}
%\newcommand{\bcm}{\fontfamily{qhv}\selectfont}
\newcommand{\bcm}{\ttfamily\selectfont}

\def\eg{\emph{e.g}\onedot} \def\Eg{\emph{E.g}\onedot}
\def\ie{\emph{i.e}\onedot} \def\Ie{\emph{I.e}\onedot}
\def\cf{\emph{cf}\onedot} \def\Cf{\emph{Cf}\onedot}
\def\etc{\emph{etc}\onedot} \def\vs{\emph{vs}\onedot}
\def\wrt{w.r.t\onedot} \def\dof{d.o.f\onedot}
\def\etal{\emph{et al}\onedot}


% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Define center-aligned and right-aligned versions of X
% \newcolumntype{Y}{>{\centering\arraybackslash}X}  % centered
% \newcolumntype{Z}{>{\raggedleft\arraybackslash}X} % right-aligned

% Check-mark, Cross-mark
\newcommand{\xmark}{\ding{55}}
\newcommand{\ccheck}{{\textcolor{checkcolor}{\large\checkmark}}}
\newcommand{\ccross}{{\textcolor{crosscolor}{\large\xmark}}}



\newcommand{\inlinecode}[1]{\colorbox[gray]{0.95}{\color{brinkpink}{\texttt{#1}}}}
% \lstdefinestyle{mystyle}{
%     backgroundcolor=\color[gray]{0.92},
%     basicstyle=\ttfamily,
%     breaklines=true,
%     % keepspaces=false,
% }
% \lstset{style=mystyle}
% \parindent=0pt
% \parskip = 0.3\baselineskip

% \textheight = 9.05 in
% \textwidth = 6.7 in
% \oddsidemargin = -0.25 in

\newcommand{\vsto}[1][3pt]{\mathrel{%
   \hbox{\rule[\dimexpr\fontdimen22\textfont2-.2pt\relax]{#1}{.4pt}}%
   \mkern-4mu\hbox{\usefont{U}{lasy}{m}{n}\symbol{41}}}}
